A Tensor Compiler for Unified Machine Learning Prediction Serving

Machine Learning (ML) adoption in the enterprise requires simpler and more efficient software infrastructure---the bespoke solutions typical in large web companies are simply untenable. Model scoring, the process of obtaining predictions from a trained model over new data, is a primary contributor to infrastructure complexity and cost as models are trained once but used many times. In this paper we propose HUMMINGBIRD, a novel approach to model scoring, which compiles featurization operators and traditional ML models (e.g., decision trees) into a small set of tensor operations. This approach inherently reduces infrastructure complexity and directly leverages existing investments in Neural Network compilers and runtimes to generate efficient computations for both CPU and hardware accelerators. Our performance results are intriguing: despite replacing imperative computations (e.g., tree traversals) with tensor computation abstractions, HUMMINGBIRD is competitive and often outperforms hand-crafted kernels on micro-benchmarks on both CPU and GPU, while enabling seamless end-to-end acceleration of ML pipelines. We have released HUMMINGBIRD as open source.

==> Makefile <==
TARGET=finetune

TEXFILE=$(TARGET).tex
TEXFILES=$(wildcard *.tex)
BIBFILES=$(TARGET).bib
FIGFILES=$(wildcard figures/*.pdf)
FIGFILES+=$(wildcard figures/*/*.pdf)
EPSFILES=$(wildcard figures/*.eps)
EPSFILES+=$(wildcard figures/*/*.eps)

MAKE_TARGET=${MAKECMDGOALS}
ifeq (${MAKE_TARGET},)
	MAKE_TARGET=${TARGET}
endif

all: ${TARGET}.pdf

${TARGET}.pdf: ${TEXFILES} ${BIBFILES} ${PKGFILE} ${FIGFILES} ${EPSFILES} ${TARGET}.bbl
	( \
	pdflatex $(TARGET).tex; \
	while grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		pdflatex $(TARGET).tex; \
	done \
	)

fig: all

figures/%.pdf: scripts/%.py scripts/common.py $(wildcard datas/%*.csv)
	if [ "$(MAKE_TARGET)" = "fig" ]; then \
		$< noblock; \
	else \
		touch $@; \
	fi


${TARGET}.bbl: ${TARGET}.bib
	pdflatex ${TARGET}.tex
	bibtex ${TARGET}
	pdflatex ${TARGET}.tex
	pdflatex ${TARGET}.tex

clean:
	rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.pdf) \
	$(TEXFILE:.tex=.thm) \
	$(TEXFILE:.tex=.bbl) \
	$(TEXFILE:.tex=.blg) \
	$(TEXFILE:.tex=.ps)


distclean: clean
	rm -f figures/*-converted-to.pdf
	rm -f figures/*/*-converted-to.pdf



==> optimizer.tex <==
% \vspace{-2mm}
%\section{Optimizations}\label{s:optimizer}
\eat{
In this section we discuss the key optimizations performed by the \system optimizer: heuristics for picking operator strategy, and runtime-independent optimizations.
Recall that, in addition to these, our approach also leverages runtime-specific optimizations at the Tensor DAG Compiler level.
We refer the interested reader to ~\cite{onnx-runtime,torchscript,tvm} for more technical details on those.
%These two types of optimizations are reminiscent of \textit{logical} and \textit{physical} optimizations in the DBMS, in a broad sense.
}

% \vspace{-2mm}


\eat{
\vspace{-2mm}
\subsection{Backend-Independent Optimizations}
\label{sec:back-ind}
We discuss four novel optimizations, which are unique to traditional ML scoring.
To the best of our knowledge, this is the first time that they are being applied in classical ML scoring. % and can be even implemented in classical ML tools.
Our approach is heavily based on the fact that, differently than training, prediction pipelines contains information that can be exploited by optimizations at compile time.

% \vspace{2mm}
\stitle{Feature Selection Push-Down.} Feature selection is a popular operation that is often used as the \textit{final featurization step} as it reduces over-fitting and improves the accuracy of the ML model~\cite{feature_selection}. 
However, during scoring, it can be pushed down in the pipeline to avoid redundant computations such as scaling and one-hot encoding for discarded features or even reading the feature at all.
This idea is similar to the concept of projection push-down in relation query processing but through user-defined table functions, which in our case are the ML operators.
For operators such as feature scaling, which performs 1-to-1 feature transformations, selection push-down can be easily done.
However, for operators such as one-hot encoding and polynomial featurization, which perform 1-to-m or m-to-1 feature transformations, the operator will have to absorb the feature selection and stop generating those features.
For example, say one-hot encoding is applied on a categorical feature column which has a vocabulary size of 10, but 4 of those features are discarded by the feature selector. In such cases, we can remove such features from the vocabulary. 
After such absorbing, it is possible that some of the input features can still be discarded as they are not used at all, which allows us to push the feature selection even further.
Note that for some ``blocking'' operators~\cite{pretzel}, such as feature normalizers, it is not possible to push-down the feature selection.

% \vspace{2mm}
\stitle{Feature Selection Injection.} Even if the original pipeline doesn't have a feature selection operator, it is possible to inject one and then push it down to avoid redundant computations. Linear models with L1 regularization (Lasso) is a typical example where feature selection is implicitly performed. 
The same idea can be extended to tree-based models to prune the features that are not used as decision variables.
In both of these examples, the ML model also has to be updated to take into account the pruned features. For linear models we prune the zero weights; for tree models, we update the indices of the decision variables.

% \vspace{2mm}
\stitle{Algebraic Rewrites.} We found opportunities to rewrite several operators that perform linear algebra operations into a single \texttt{GEMM} operation.
Consider a pipeline that trains a logistic regression model and has feature scaling and matrix decomposition (e.g., PCA) as the featurization steps.
It is algebraically represented in Eq.~\ref{eq:algebraic_rewrite}-LHS. 

\vspace{-2mm}
\begin{multline}\label{eq:algebraic_rewrite}
    \texttt{sigmoid}\bigg(\Big(\big(\frac{X - \alpha}{\beta}\big) \cdot W_{PCA} \Big) \cdot W_{LR} + B_{LR} \bigg) \\
    = \texttt{sigmoid}(X\cdot W + B)
\end{multline}

Notice that parentheses in Eq.~\ref{eq:algebraic_rewrite}-LHS capture the order in which the operators were trained and it requires performing 5 tensor operations: 2 element-wise ops for scaling; two \texttt{GEMM} ops for matrix decomposition and logistic regression; and a final \texttt{sigmoid} op for logistic regression.
It is possible to use linear algebra properties and represent the same pipeline using two ops as shown in RHS, where tensor $W$ and $B$ can be pre-computed and used during scoring.
These kinds of patterns are in fact very common in classical ML; any subset of scaling, matrix decomposition, and linear models constitutes such patterns.
However, they do not appear in DNNs due to the use of non-linear transformations and hence most tensor runtime optimizers are oblivious of these opportunities.
%\system's optimizer has a roster of such patterns and checks for potential rewrites during optimization.

% \vspace{2mm}
\stitle{Batching Stacked Models.} Recall that in Section~\ref{ss:tree_compilation}, we batched the tensors from all trees into single tensors and performed batched tensor operations.
Alternatively, we could have stored them separately and invoke tensor operations on each tree.
Though this would yield the same result it will be highly inefficient due to two reasons: (1) high operator invocation overhead and (2) high memory access overhead (due to multiple reading of the input tensor $X$).
It is possible to apply the same batching optimization across multiple ML operators.
Consider a stacked ML model that is composed of logistic regression, linear SVM, and Bernoulli Naive Bayes models.
While these models are conceptually different during scoring all three of them are essentially performing a \texttt{GEMM} operation.
Thus, it is possible to batch them together into one \texttt{GEMM} operation to reduce overheads.
Efficiently finding this type of graph substitutions in an arbitrary tensor computation DAG is still an active area of research~\cite{taso}; hence not supported by many DNN runtimes.
On the other hand, \system implements few patterns as the one above, directly over traditional ML operators. %and triggers batching rewrites.
}


% In Pipeline 1, before feeding the features to the linear model, there is a feature selection operator to discard not useful features.
% However, during scoring time this operator can be pushed down, similarly to projection push-down in databases.
% This avoids redundant computations such as scaling and one-hot encoding for discarded features, or even reading the feature at all.
% For operators such as feature scaling, which performs 1-to-1 transformations, selection push-down can be easily implemented.
% However, for 1-to-n and n-to-1 operators such as one-hot encoding and polynomial featurizer, the operator will have to absorb the feature selection.
% After absorbing, it is possible that some of the original features can still be discarded as they are not used.
% This allows us to push the feature selection even further.
% Note that for some operators, such as feature normalizers, it is not possible to push-down the feature selection.

% \vspace{2mm}
% \stitle{Feature Selection Injection.} Even if the original pipeline doesn't have a feature selection operator, it is possible to inject one and then push it down to avoid redundant computations. L1 regularization (Lasso) is a typical example where feature selection is implicitly performed.
% The same idea can be extended to tree-based models to prune the features that are not used as decision variables.

% \vspace{2mm}
% \stitle{Algebraic Rewrites.} This includes operator fusion and operator batching optimizations.
% For example the scaling operator and logistic regression model in the pipeline shown in \autoref{fig:optimizations} (A) can be merged into one operator which performs a single generic matrix multiplication (GEMM) operation.
% Similarly, feature scaling + matrix decomposition (e.g., PCA), matrix decomposition + linear models, and feature scaling + matrix decomposition + linear model can also be fused into one GEMM operation. Note that these are very common operator combinations in classical ML pipelines.
% Furthermore, consider a stacked ensemble model which is composed of logistic regression, linear SVM, and a Naive Bayes models.
% While these models are conceptually different, during scoring time all three of them are essentially performing a GEMM operation.
% Thus, it is possible to batch them together into one GEMM operation in order to reduce the overheads.

% \vspace{2mm}
% \stitle{Batching Ensemble Models.}



% \KK{I think some reorganization is needed here. I would suggest to mention the translation from traditional ML to DNNs first, and then the optimizations. Also, it is not clear if these optimizations are required to perform the translation or they are completely complimentary. And are these optimizations enabled by HB or are they optimizations that you would do to any traditional ML pipeline? If it's the latter, we need to discuss what exactly is the purpose of this section. Is it, for instance, that they are not required but that without them you cannot get good performance?}
% \mi{Agreed. With more space we should give a proper introduction to the system and explain more in detail how the compilation process work. I think that some optimizations are specific to the approach (e.g., tree optimizations) but some of them are more generic and can be applied elsewhere, like the feature selection stuff or the batching of linear with scaler. Yes we should be more specific on this.}

% \system's optimizations can be broadly classified into three categories:

% \KK{Rereading this, let's discuss about how to reorganize it. The current section makes me think that you are describing the "optimizer" in the architecture figure, but in fact, there are optimizations happening after/during the DAG generation too (e.g., cross-operator and runtime optimizations). Also, I would make the generation of NN based on trees a separate section. These optimizations that you describe here are important performance-wise but not as interesting as the NN generation. They are more to say "dont just naively generate NNs).}

% \begin{figure*}[ht]
% % \vspace{-3mm}
% \centering
% \includegraphics[width=0.9\textwidth]{figures/pipeline_optimizations.pdf}
% \caption{\system~ optimizations. (A) Feature selection push-down (DAG transformation), (B) Fusing feature scaling with logistic regression (cross-operator optimization). \CC{We should split/reorganize this figures a bit.}}
% \label{fig:optimizations}
% % \vspace{-3mm}
% \end{figure*}

% \vspace{2mm}
% \stitle{DAG Transformations.} In classical ML pipelines there are opportunities to optimize the end-to-end pipeline through  transformation rules, which are only applicable in the \emph{scoring} setting. \KK{I think this comment (that they are only applicable in scoring) makes a lot of sense if one knows that there is HB for training, but here it needs some more explanation.}
% \mi{Yep. We were thinking about structuring the paper such that upfront we explain that classical ml can be compiled either into differentiable and non-differentiable operations. Using non-diff operations we can be more efficient.}
% For example consider the transformed version of the Pipeline 1 of \autoref{fig:pipeline} shown in \autoref{fig:optimizations} (A).
% In Pipeline 1, before feeding the features to the linear model, there is a feature selection operator to discard not useful features.
% However, during scoring time this operator can be pushed down, similarly to projection push-down in databases.
% This avoids redundant computations such as scaling and one-hot encoding for discarded features, or even reading the feature at all.

% For operators such as feature scaling, which performs 1-to-1 transformations, selection push-down can be easily implemented.
% However, for 1-to-n and n-to-1 operators such as one-hot encoding and polynomial featurizer, the operator will have to absorb the feature selection.
% After absorbing, it is possible that some of the original features can still be discarded as they are not used.
% %This allows us to push the feature selection even further.
% Note that for some operators, such as feature normalizers, it is not possible to push-down the feature selection.

% Even if the original pipeline doesn't have a feature selection operator, it is possible to inject one and then push it down to avoid redundant computations. L1 regularization (Lasso) is a typical example where feature selection is implicitly performed.
% The same idea can be extended to tree-based models to prune the features that are not used as decision variables.

% \vspace{2mm}
% \stitle{Cross-operator Optimizations.} Our approach also opens up the opportunity to perform several cross-operator optimizations. This includes operator fusion and operator batching optimizations.
% For example the scaling operator and logistic regression model in the pipeline shown in \autoref{fig:optimizations} (A) can be merged into one operator which performs a single generic matrix multiplication (GEMM) operation.
% Similarly, feature scaling + matrix decomposition (e.g., PCA), matrix decomposition + linear models, and feature scaling + matrix decomposition + linear model can also be fused into one GEMM operation. Note that these are very common operator combinations in classical ML pipelines.
% Furthermore, consider a stacked ensemble model which is composed of logistic regression, linear SVM, and a Naive Bayes models.
% While these models are conceptually different, during scoring time all three of them are essentially performing a GEMM operation.
% Thus, it is possible to batch them together into one GEMM operation in order to reduce the overheads.

% \vspace{2mm}
% \stitle{Runtime Optimizations.} Our compilation approach enables us to leverage runtime-dependant optimizations such as low-precision scoring (e.g., in TensorRT) and optimized kernel generation (e.g., TVM) which are not possible or hard to implement otherwise.

% \vspace{2mm}
% \stitle{Cost-based compilation target selection.}
% When compiling classical ML pipelines, for a given high-level operator there can be more than one compilation target.
% \gi{Also it looks like for given a DAG of operators, there can be multiple targets. Simple example: let's say we have a ensemble of logistic regression and linear SVM, and they use different features by applying different feature selection ops. In this case, we can either 1) incorporate redundancy (select the union of features used by logistic regression and SVM) and batch the two GEMM operators or 2) do not batch GEMMs.}
% For example, in the case of decision tree-based models, \system currently supports three possible compilation strategies.
% In practice, none of the strategies are globally optimal, but instead they are all applicable in different situations based on the input model structure.
% For example, as we will see in the next section, one strategy \system uses to implement tree scoring is to compute all internal decisions at once~\cite{finetune}. 
% Clearly, as the size of the decision trees get bigger, this strategy will be significantly inefficient due to redundant computations.
% With this strategy we in fact perform $O(2^h)$ ($h$ is the height of the tree) computations whereas the original algorithmic operator needs to perform only $O(h)$ comparisons.
% Nevertheless, the above compilation strategy implement tree traversal as GEMM operations, therefore up to a certain depth level this strategy can be actually optimal performance-wise on modern hardware, where GEMM operations can run highly efficiently.
% %However, with modern hardware, generic matrix multiplication (GEMM) can be run highly efficiently, therefore up to a certain depth level this strategy can be actually optimal performance-wise.
% The exact crossover point where one strategy outperforms the others is determined by the characteristics of the execution engine and the available hardware.
% For instance, we have experimental evidences showing that the above strategy performs better over shallow trees ($h \leq 3$), whereas tree-traversal-based strategies perform better over deep trees.
% %\mw{This leaves some details to be desired.}
% %\mi{Well, we haven't figured this part yet. We have empirical evidence for this, but not yet a cost base model. We will have it for the long version.}
% %\mw{Do we have stats that at least proof the basic point that there is a crossover point?}
% %\mi{we know that with different tree depths one strategy outperform the other. Basically there is no strategy always winning. I think we need to do some additional experiment do find a cross point (at least for trees) and then generalize over using a cost model.}
% %\mw{Maybe just mention that we have done preliminary experiments which showed this behavior?}
% Thus, in \system~ we use a cost model for compilation target selection, reminiscent to relational data management systems.
% Next we give details on the strategies \system uses to compile tree-base models into tensor computations.
